Link Prediction by De-anonymization: How We Won the Kaggle Social Network Challenge

This paper describes the winning entry to the IJCNN 2011 Social Network Challenge run by Kaggle.com. The goal of the contest was to promote research on real-world link prediction, and the dataset was a graph obtained by crawling the popular Flickr social photo sharing website, with user identities scrubbed. By de-anonymizing much of the competition test set using our own Flickr crawl, we were able to effectively game the competition. Our attack represents a new application of de-anonymization to gaming machine learning contests, suggesting changes in how future competitions should be run. We introduce a new simulated annealing-based weighted graph matching algorithm for the seeding step of de-anonymization. We also show how to combine de-anonymization with link prediction---the latter is required to achieve good performance on the portion of the test set not de-anonymized---for example by training the predictor on the de-anonymized portion of the test set, and combining probabilistic predictions from de-anonymization and link prediction.

==> acks.tex <==
\section*{Acknowledgments}

We would like to thank Yong J Kil and Chris Li for their assistance and many helpful discussions. We are also very grateful to the competition organizers Dirk Nachbar, Anthony Goldbloom, Jeremy Howard, and the collegial atmosphere shared by our fellow Challenge participants.
Elaine Shi would like to thank Srinath Sridhar
and Chengwen Chris Wang for their helpful consultations.


==> conc.tex <==
\section{Conclusions \& Open Problems}

We have described a de-anonymization attack on link prediction contests, which was used in the winning entry to the IJCNN 2011 Social Network Challenge run by Kaggle.com.

While the competition dataset was scrubbed of user identities, the revelation that the graph had been obtained by crawling Flickr proved sufficient for our attack. Using our own crawl of Flickr, we were able to successfully de-anonymize 64.7\% of the test edge-set. And by training a Random Forest classifier on standard link prediction features of the training plus de-anonymized test sets, we were able to achieve a winning test AUC of 0.981.

We made several technical contributions in developing our attack. We introduced a new approach to seed-identification, which is applicable to weighted graph matching more generally. We also described how to combine the results of de-anonymization and link prediction: the link prediction training set is augmented by the partially de-anonymized test set, and probabilistic predictions from both processes are used together.

The success of our attack on the Social Network Challenge has important consequences for the future of such contests. We have argued that forbidding outside data sources and requiring source code submissions may not eliminate the problem. Ruling out de-anonymization while preserving meaningful utility remains an open question. 

Identifying the source of anonymized social graph data is also an interesting research direction, although it is likely that global characteristics such as joint degree distribution would suffice to  differentiate online social networks in a straightforward manner.

While previous work on social network link prediction mainly 
exploits the structure of the graph itself~\cite{Liben-Nowell:2003:LPP:956863.956972,MurataM08,Corlette2010},
our work suggests a promising new direction, 
namely, incorporating the vast amount of information publicly available on the web.
Our de-anonymization approach may be regarded an extreme case;
more generally, it may be possible to leverage statistical or aggregate information gleaned from the web to improve link prediction.
%of leveraging outside information in link prediction.  In real-world settings, one may need to perform link prediction for a social graph $G$, with the knowledge of several other social graphs $G_1, \ldots, G_k$. In these cases, direct deanonymization would be less successful, but it would be interesting to seek other means to incorporate such outside information   in the task of link prediction.
It would also be interesting to investigate how to incorporate semantic information attached to nodes and edges into link prediction. 



==> discuss.tex <==
\section{Discussion}\label{sec:discuss}

%\todo{One paragraph explaining that we're morally clean because we let the organizers know before the contest.}

Our primary goal for participating in the Challenge was to raise attention to the
ever-present possibility of de-anonymization in such contests.
More broadly one might ask whether contests should discourage the use of
outside information in general---trading off the benefits of leveraging outside
information to genuinely improve the outcomes of data mining, and preventing
cheating---and what technical or policy means could be used to limit such
information.

In addition to undermining the aim of the contest, which was to advance the
state-of-the-art in machine learning, de-anonymization also has privacy implications
(although these did not arise in this contest). For these reasons, it is important 
to think about how to prevent de-anonymization in future contests.
One factor that greatly affects both risks---in opposite directions---is whether the underlying data is already publicly available. If it is, then there is likely no privacy risk; however, it furnishes a ready source of high-quality data to game the contest. On the other hand, if the data is not public, then it can only be exploited by cross-referencing it through de-anonymization with another dataset of the same type (or with some of the same attributes) that {\em is} public.\footnote{For example, Narayanan and Shmatikov were able to re-identify anonymized records in the Netflix Prize dataset with user accounts on IMDb via their public movie reviews \cite{netflix}.} While this presents a significant privacy risk, imperfect correlation between the two datasets makes it unclear whether there is a threat to the fidelity of the contest.

Focusing on the threat of de-anonymization to the contest, incorporating a restriction on the use of external data in the rules is a necessary step, but arguably insufficient, since less scrupulous contestants may attempt to apply de-anonymization anyway. We can see two possible ways to combat this threat. The first is the approach taken by the Netflix Prize---require teams qualifying for prizes to produce source code and human-readable descriptions of algorithms.  The Netflix Prize stipulated that the verification process would ``ensure that the provided algorithm description and source code could reasonably have generated the prediction sets submitted.''

The loophole in this approach is the possibility of overfitting. While source-code verification would undoubtedly catch a contestant who achieved their results using de-anonymization alone, the more realistic threat is that of de-anonymization being used to bridge a small gap. In this scenario, a machine learning algorithm would be trained on the {\em test set}, the correct results having been obtained via de-anonymization. Since successful ML solutions are composites of numerous algorithms, and consequently have a huge number of parameters, it should be possible to conceal a significant amount of overfitting in this manner.

Another approach is to attempt to prevent the possibility of de-anonymization. This is a daunting task: a long line of research has demonstrated the feasibility of de-anonymization on various datasets \cite{sweeney,sweeney-malin,grouplens,homer,netflix,ns09,locationpairs,writeprints} and theoretical evidence exists for the impossibility of de-anonymization of high-dimensional data \cite{curse}.

%With graph data, one could try to modify the released graph so as to make seed identification hard; our experience suggests that once enough seeds are found, the propagation algorithm is highly robust. While our seed-identification task was made somewhat difficult by the fact that only a fraction of nodes were included {\em as sources} in the Kaggle graph, it was aided by the fact that no nodes were excluded {\em as sinks} of edges. It is not clear if seed identification would succeed if the released graph were additionally restricted in this manner. Our intuition, however, is that it is simply a matter of coming up with a sufficiently clever seed-identification heuristic tuned to the sanitization mechanism.

Several papers have claimed to provide k-anonymity, or variants thereof, for graphs \cite{kanon1,kanon2,kanon3,kanon4}. These have only been evaluated against graphs with a small number of nodes and small average degree. Further, they only consider the threat of adversaries with restricted types of auxiliary information, which in particular does not include {\em global} information such as another graph that is structurally related to the target graph. For these reasons we do not believe these techniques are effective ways to anonymize social networking graphs.

Finally, differential privacy offers a potential method to bypass the need for anonymization \cite{dp-survey}. McSherry and Mironov show how the Netflix Prize contest could have been run by releasing a differentially private dataset (primarily, a sanitized item-item covariance matrix) instead of raw user data \cite{dp-netflix}. 
The drawbacks of this approach are that it would restrict 
the class of machine learning algorithms, and may require a shift 
from the ``release-and-forget'' model to an online privacy-preserving computation model, especially due to the difficulty of 
generating synthetic datasets that preserve differential
privacy~\cite{UllmanV10}.
Nevertheless, differential privacy remains essentially the only 
mathematically sound methodology for provably resisting de-anonymization.

%\todo{Address the McSherry and Mironov paper as well as papers claiming k-anonymity for graphs.}

%Finally, there is the approach of releasing differentially private data. 

%\ben{May be interesting to discuss the concept of cheating, and using outside data in competitions. As Elaine nicely put it, it should be fine to use aggregate statistics from outside data but maybe not each individual datum... almost smells like differential privacy to me...}


==> intro.tex <==
\section{Introduction}

\PARstart{K}{aggle.com}---a platform for machine learning
competitions---ran the IJCNN 2011 Social Network Challenge for 9 weeks from
Nov 8, 2010 through Jan 11, 2011~\cite{kaggle-challenge}. 
The goal of the Social Network Challenge was to promote research on
link prediction. The contest dataset was created by crawling a large online
social network and partitioning the obtained edge set into a large training
set and a smaller test set of edges augmented with an equal number of
fake edges. 
Challenge entries were required to be probabilistic predictions 
on the test edge set.
Node identities in the released data were obfuscated to prevent cheating. 

Of the 119 teams competing in the link prediction task, we placed
first by de-anonymizing a large portion of the test set and applying a
combination of standard machine learning techniques on the remainder. While
our participation in the challenge raised obvious questions on the propriety
of our methods, our goal was to raise attention to the ever-present
possibility of de-anonymization in such contests.\footnote{Once we had established a clear lead on the public leaderboard, we contacted the organizers to inquire about how to proceed, offering to withdraw if that was deemed to be best. Happily, the organizers found our method acceptable, and noted its novelty.}

The contributions of this paper are three-fold. First we demonstrate that
partial crawls of a large real-world online social network can be
effectively de-anonymized, whereas prior work studied 
de-anonymizing complete snapshots of social
networks~\cite{ns09}. We achieve this by focusing on nodes with high in-degrees
for ``seeding'' the de-anonymization process.  
As we explain in Section \ref{sec:seed-identification}, 
the set of high in-degree nodes is (approximately) preserved even in a snapshot
obtained from a partial crawl.

%While the high-degree nodes---the ``seed'' nodes matched in the first step of de-anonymization---may not be crawled in the target graph, it is likely that a subset of their incoming neighbors are crawled, leading to accurate estimates of relative in-degree's. 


Second, we formulate seed identification---the first step of de-anonymization---as a combinatorial optimization problem, specifically {\em weighted graph matching}, in contrast to the pattern search approaches of \cite{wherefore} and \cite{ns09}. We then show how to use simulated annealing to solve this problem. Since our formulation makes no assumptions specific to the de-anonymization context, our solution is broadly applicable to the weighted graph matching problem.

%Second, we propose a new method for iteratively growing the de-anonymization process' graph matching using simulated annealing. \todo{more?}. This approach can be applied to any de-anonymization scheme and is not restricted to link prediction.

Third, our winning entry, which yielded a combined test Area Under Curve (AUC)
of 0.981, made use of a novel combination of standard link prediction with
de-anonymization to game a popular link prediction contest. Moreover the
link prediction component of our entry was advantaged by training on the
de-anonymized portions of the test set. While previous applications of
de-anonymization have been to privacy attacks \cite{sweeney, netflix},
to the best of our knowledge this is the first application of
de-anonymization to gaming a machine learning contest.

The success of our approach has important consequences for future machine
learning contests particularly in social network analysis.
We argue that while appropriate contest rules should be used to disincentivize gaming
through de-anonymization, technical measures to detect gaming 
are unlikely to be foolproof.  Releasing useful social network graph data that is
resilient to de-anonymization remains an open question.



==> related.tex <==
\section{Related work}
\label{sec:related-work}

{\bf Link prediction.} 
Several prior works study the problem of social network 
link prediction through graph structural analysis~\cite{Liben-Nowell:2003:LPP:956863.956972,MurataM08,Corlette2010}.
Notably, our link prediction algorithm and those of other
top teams leveraged 
several features proposed by 
Liben-Nowell and Kleinberg~\cite{Liben-Nowell:2003:LPP:956863.956972}.
Unfortunately, the large size of the graph precluded 
the use of all features 
described therein when running
on a commodity computer~\cite{2ndplace}.

Other teams in the contest achieved impressive results using pure link prediction. In particular, Cukierski, Yang, and Hamner finished second, and their link prediction algorithm involved running Random Forests over $94$ selected features~\cite{2ndplace} and achieved an extraordinary AUC of $0.969$.


{\bf Social network de-anonymization.} Backstrom et al.~\cite{wherefore} showed how to de-anonymize specific nodes and edges in a social network by searching for patterns in subgraphs of small size (logarithmic; in practice, around 7 nodes). Narayanan and Shmatikov studied de-anonymization of a social network on a large scale by using a different social network as auxiliary data~\cite{ns09}.

{\bf Inexact graph matching} is a well-studied problem that arises in diverse applications, primarily image recognition. Bengoetxea's thesis \cite{igm-thesis} surveys numerous approaches to solving it, including genetic algorithms, simulated annealing, expectation maximization, decision trees, and neural networks. It is possible that some of these techniques would extend to weighted graph matching.

Weighted graph matching has been studied in~\cite{wgm-eigen, wgm-lp}. These papers are concerned with finding the optimal solution rather than an approximation, and therefore their techniques only work for small numbers of nodes.


